Threshold Matters in WSSS: Manipulating the Activation for the Robust and Accurate Segmentation Model Against Thresholds

Weakly-supervised semantic segmentation (WSSS) has recently gained much attention for its promise to train segmentation models only with image-level labels. Existing WSSS methods commonly argue that the sparse coverage of CAM incurs the performance bottleneck of WSSS. This paper provides analytical and empirical evidence that the actual bottleneck may not be sparse coverage but a global thresholding scheme applied after CAM. Then, we show that this issue can be mitigated by satisfying two conditions; 1) reducing the imbalance in the foreground activation and 2) increasing the gap between the foreground and the background activation. Based on these findings, we propose a novel activation manipulation network with a per-pixel classification loss and a label conditioning module. Per-pixel classification naturally induces two-level activation in activation maps, which can penalize the most discriminative parts, promote the less discriminative parts, and deactivate the background regions. Label conditioning imposes that the output label of pseudo-masks should be any of true image-level labels; it penalizes the wrong activation assigned to non-target classes. Based on extensive analysis and evaluations, we demonstrate that each component helps produce accurate pseudo-masks, achieving the robustness against the choice of the global threshold. Finally, our model achieves state-of-the-art records on both PASCAL VOC 2012 and MS COCO 2014 datasets.

==> tab/lc_accuracy.tex <==
\begin{table}
\centering %< auto-adjusts font size to fill line
{\small
\begin{tabular}{@{}ccc@{}}

\toprule
 & AMN & \multirow{2}{*}{AMN}\\
 & w/o LC & \\
\midrule
Accuracy & 19.7\% & 96.2\% \\
\bottomrule
\end{tabular}
}
\caption{
Accuracy of predicted class from AMN on PASCAL VOC 2012 train set. The activation corresponding to the given label was successfully induced by LC. 
}
\label{tab:lc_accuracy}
\end{table}


